Data-Driven Discovery of the Origins of UV Absorption in Alpha-3C Protein

Over the last decade, there has been a growing body of experimental work showing that proteins devoid of aromatic and conjugated groups can absorb light in the near-UV beyond 300 nm and emit visible light. Understanding the origins of this phenomena offers the possibility of designing non-invasive spectroscopic probes for local interactions in biological systems. It was recently found that the synthetic protein {\alpha}3C displays UV-vis absorption between 250-800 nm which was shown to arise from charge-transfer excitations between charged amino acids. In this work, we use data-driven discovery to revisit the origins of these features using molecular dynamics and excited-state simulations. Specifically, an unsupervised learning approach beginning with encoding protein environments with local atomic descriptors, is employed to automatically detect relevant structural motifs. We identify three main motifs corresponding to different hydrogen-bonding patterns that are subsequently used to perform QM/MM simulations including the entire protein and solvent bath with the density-functional tight-binding (DFTB) approach. Hydrogen-bonding structures involving arginine and carboxylate groups appear to be the most prone to near-UV absorption. We show that these features are highly sensitive to the size of the QM region employed as well as to the inclusion of explicit solvation underscoring the limitations of using gas-phase cluster models.

==> main-questions.tex <==
\section{Hhm Charge Transfer Excitations from TDDFTB (or TDDFT) Calculations?!}
\begin{itemize}
    \item We are using long range corrected slatter coster parameters
    \item We bench marked our results by doing TDDFT with CAM-B3LYP functional
\end{itemize}

\subsection{Why do people get suspicious when presented CT results obtained using DFT or anything related to it? What approximate CT energies better?}
\textbf{Something about the functional?}

Let us go slowly from Hartree-Fock to DFT and DFTB, seeing how they approximate the quantum mechanical energy.

\subsection{Hartree-Fock}
\begin{equation}
    \left[ -\dfrac{\Bar{h}^2}{2m}\xrightarrow{\delta}^2 + V^{ext} + V^H + V^X \right] \phi_k (\xrightarrow{r}) = \epsilon_k \phi_k(\xrightarrow{r})
\end{equation}
$H^{HF}$ is 
\begin{itemize}
    \item single particle 
    \item acts in hilbert space of spin-orbitals (single particle orbitals)
    \item self-consistent (depend on its own eigen functions)
    \item eigenvalues of $H^{HF}$, $\epsilon_i$ are NOT energies of electronic system
    $$H^{HF}|\phi_i> = \epsilon_i|\phi_i> \qquad H_e|\Phi> = E_I|\Phi>$$
    $$E_0 ~ E^{HF}$$ (always greater than $E_0$, it is its upper bound)
\end{itemize}
So it is tempting to call (let's say in a 6 valence electrons system) the difference between $\epsilon_3$ and $\epsilon_4$ a band gap, but it is VERY WRONG. $\epsilon_s$ are diagonals of Langrange Multipliers NOT energy levels. So it gives wrong energy values, with like 5 or 10 times the real (exp) band gap.
DFT also do the same, in a sense that it arrives on a similar thing, some kind of single particle Hamiltonian which will have its own eigen values \hdots but DFT often values are better. 





\section{Why Does Removing Water Molecules from QM Region Red-Shifts the Absorption instead of Blue-Shifting It?}
In QM/MM set-up: removal of water in QM region blue-shifts the absorption spectrum
In vacuum: removal of water in the QM cluster red-shifts the absorption spectrum

\section{What Lead to these Huge Red-shifts}

We tried couldn't see relevant structural motifs the
